Studies of low-energy effective actions in supersymmetric field theories

This thesis examines low-energy effective actions of supersymmetric quantum field theories. These actions contain information about the low-energy field content and dynamics of quantum field theories and are essential for understanding their phenomenological and theoretical properties. In chapters 2 to 5, the covariant background field method is used to investigate quantum corrections to sectors of a variety of supersymmetric field theories at 1 and 2 loops. We start by looking at the background field quantisation of a general N=1 super-Yang-Mills theory, rederiving the well-known 1 loop finiteness conditions. This is followed by a reexamination of the effective potential of the Wess-Zumino model, focusing on a derivation of the full auxiliary fields' potential. Next, the 2 loop Euler-Heisenberg effective action is constructed for N=1 supersymmetric quantum electrodynamics; its renormalisation properties and self-dual limit are studied. The final action studied is the 2 loop Kahler potential for beta-deformed N=4 super-Yang-Mills. This sector is purely a product of the deformation and its finiteness is demonstrated in a general background before examining two special cases. Chapter 6 studies spontaneously broken supersymmetry and the pure Goldstino action. A general approach to constructing explicit field redefinitions is used to relate all known models of the Goldstino and to study their nonlinear supersymmetries. This approach is also used to construct the most general pure Goldstino action and to examine its supersymmetry transformations. Finally, a new embedding of the Goldstino into a complex linear superfield is presented. Its interactions to matter and gravity are examined and compared to existing Goldstino superfield constructions.

==> ASect_CoupledMCL.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Constrained complex linear superfield with interactions}%
\label{CoupledMCLConstraints}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In section \ref{ssect:couplings}, we discussed how the constrained
complex linear superfield realization of the Goldstino could be coupled
to a matter sector.
One way was to generalize the standard interactions of chiral and complex linear
superfields by using the modified constraints 
(\ref{coupled mCL 1}, \ref{coupled mCL 2}).
In this appendix we solve those constraints and investigate the resultant
component supersymmetry transformations and component action.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The constraints}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We start off with a constrained complex linear superfield $\S$
interacting with some chiral superfield $X$:
\begin{align}
\label{eqn:mCLConstr1}
 	-\frac14 \Db^2 \S &= X\,, & {\bar D}_\da X &= 0\,,  \\
	\S^2 &= 0\,,& -\frac14 \S\Db^2D_\a\S &= X D_\a\S\, .
\label{eqn:mCLConstr2}
\end{align}
The first line contains the standard constraints for interacting complex linear 
and chiral superfields \cite{Deo1985}.
The second line is what makes $\S$ the Goldstino superfield.
The superfield $X$ should have a nonvanishing vacuum expectation value
and is in general of the form
$X = f + G_1(\F) + G_2(\F) \tr(W^\a W_\a)$,
where $\F$ are some chiral matter superfields and $W_\a$ is the field
strength of a vector multiplet.

We use the component projections (that match those of section \ref{sect:mCL})
\begin{gather}%\label{}
	\S| = \f\,, 			D_\a\S| = \j_\a\,, 
	\Db_\da\S| = \sqrt{2}\bar\r_\da\,, 					\\\non
	-\frac14D^2\S| = F\,, 	D_\a\Db_\da\S| = U_\ada\,,
	-\frac14D^2\Db_\da\S| = \bar\c_\da\,,				\\\non
	-\frac14\Db^2\S| = X| = x\,,
	-\frac14D_\a\Db^2\S| = D_\a X = \vf_\a\,, 			\\\non
	\frac1{16}D^2\Db^2\S| = -\frac14 D^2 X| = \dsF\ .
\end{gather}
When $X = f$ (so that $\vf_\a=\dsF=0$), the analysis has to reduce to
that of subsection \ref{ssect:Constraints}.

The final solutions to the constraints 
(\ref{eqn:mCLConstr1},\ref{eqn:mCLConstr2}),
which can be compared with \eqref{solns-to-both-constraints}, 
are
\begin{align}\label{eqn:mCLConstrSolns}
	x \phi &= \frac{1}{2}\bar\r^2\, ,\qquad 
	x \tilde{U}_{\alpha \db}=-2\rmi \left(\pd \bar\r\right)_\a
		\bar\r_\db+\sqrt{2}\vf_\a\bar\r_{\db}\,, \non\\\non
	x^2 \psi_\a &= \frac{1}{2}\bar\r^2
		\left(-\rmi \sqrt{2}\left(\pd \bar\r\right)_\a+\vf_\a\right) \,,\\ 
	x^3 F& = \bar\r^2 \left(\pd^a\bar\r\st_{ab}\pd^b\bar\r
		+\frac{\rmi}{2\sqrt{2}}\vf \pd \bar\r
		+\frac{1}{2}x \dsF\right)\,, \\\non
	x^2\overline{\tilde{\chi }}_{\db} 
		&=-\frac1{\sqrt{2}}\left(\left(\pd_b\bar\r\st^a\s^b\bar\r\right)\pd_a\bar\r_\db
		+\left(\pd_a\bar\r\st^a\s^b\pd_b\bar\r\right)\bar\r_{\db}
		+\frac{1}{2}\left(\square \bar\r^2\right)\bar\r_{\db}\right) \\\non
		&-\rmi \left(\vf \s^a\bar\r\right)\pd_a\bar\r_{\db} 
		+\frac\rmi4\pd_{\db}^\a\left(\bar\r^2\vf_\a\right)
		+\sqrt{2}x \dsF\bar\r_{\db}
		+\sqrt{2} \left(x^{-1}\pd_ax\right)
		\left(\pd^a\bar\r^2\right)\bar\r_{\db}\ .
\end{align}

{\bf TODO: copy some of the derivation and discussion 
     of this from my \emph{Mathematica} notebook... }%TODO


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Supersymmetry transformations}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The Goldstino $\bar\r_\da$  inherits its supersymmetry transformation from 
the complex linear superfield
\begin{align}%\label{}
	\sqrt2\d_\x\bar\r_\da 
	&= \Db_\da\d_\x\S|  			\\ \non
	&= 2\bar\x_\da x + x^{-1}\big(2\rmi(\x\s^a\bar\r)\pd_a\bar\r_\da
	+ \rmi\bar\r^2\x^\a\pd_\ada\log(x) + \sqrt2(\x\j)\bar\r_\da\big)\ .
\end{align}
The components of the chiral superfield transform as normal
\begin{align*}%\label{}
	\d_\x x = \x\j\,, \quad
	\d_\x\j_\a = 2\x_\a \dsF - 2\rmi\bar\x_\db\pd_a^\db x\,,\quad
	\d_\x \dsF = \rmi(\bar\x\pd\j)\ .
\end{align*}
It is a straightforwad, but tedious exercise to check that these transformations
give the supersymmetry algebra.

What's interesting about these supersymmetry transformations 
compared to the canonical approach to nonlinear supersymmetry, 
is that the matter fields transform linearly like there was no Goldstino, 
while the Goldstino transforms into a mix of itself and the matter fields.  
%Although, this is no longer true after the matter auxilary fields are removed.

Using these supersymmetry transformations we can construct 
a Samuel-Wess type superfield. Define
\begin{align}%\label{}
	\bar\X_\da(x,\q,\bar\q) = \rme^{\d_\q}\bar\r_\da(x)\ .
\end{align}
This is a constrained superfield satisfying constraints
that are a generalization of (\ref{SW_Constraint1}, \ref{SW_Constraint2}):
\begin{align}%\label{}
	D_\a\bar\X_\db &= 2^{-1/2}X^{-1} \big(2\rmi\bar\X^\da \pd_\ada\bar\X_\db
		+ \rmi\bar\X^2\pd_{\a\db}\log(X) 
		+ 2^{1/2}(D_\a X)\bar\X_\db\big)\,, \non\\
	\Db_\da\bar\X_\db &= 2^{1/2} \eps_\dadb X\ .
\end{align}
The superfield $\bar\X_\da$ is a description of the interacting Goldstino 
that is equivalent as the original constrained complex linear superfield $\S$.
In fact, we can reconstruct the latter %constrained complex linear superfield 
as
\begin{align*}%\label{}
	\S = \frac12 X^{-1} \bar\X^2\ .
\end{align*}
It is not hard to %double 
check that this construction satisfies the 
original constraints (\ref{eqn:mCLConstr1}, \ref{eqn:mCLConstr2}).
It also yields the same component projections \eqref{eqn:mCLConstrSolns}
and the first term, at least, is easy
\begin{align*}%\label{}
	\f = \S| = \frac12X^{-1}\bar\X^2| = \frac12 x^{-1}\bar\r^2\ .
\end{align*}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The action}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The superfield action consists of 
a pure matter part and a Goldstino/matter part,
$S[\S,\bar\S,X,\bar{X}] = S[X,\bar{X}] + S[\S,\bar\S]$.
%
When the nonlinear constraints are enforced, 
the latter %action $S[\S,\bar\S] = -\intz \bar\S \S$ 
decomposes into a pure Goldstino part, 
equal to the Samuel-Wess (chiral AV) action, 
and a part that contains the Goldstino/matter coupling terms.
%\begin{align*}%\label{}
%	S[\S,\bar\S,X,\bar{X}] = S[X,\bar{X}] + S[\S,\bar\S] 
%	= S[X] + S_\text{SW}[\S] + S_\text{int}[\S]\ .
%\end{align*}

Projecting out the components of the action
\begin{align*}%\label{}
	S[\S,\bar\S] = -\intz \bar\S \S\,,
\end{align*}
and using the contraint solutions \eqref{eqn:mCLConstrSolns} yields
\begin{align}%\label{} 
\!	S[\S,\bar\S] %&= -\intz \bar\S \S  \allowdisplaybreaks\non\\ \non
	&= -\intx \Bigg[|x|^2
	+ \frac{\rmi}{2} \r \oLRa\pd \bar{\r} %+ \frac{\rmi}{2} \bar{\r}\pd\r 
	+\frac{1}{4}|x|^{-2}\big((\pd_a\r^2)(\pd^a\bar\r ^2)
		+4 (\r \pd \bar\r)(\bar\r \pd \r)\big) \non\\\non
	&-\frac{1}{4}|x|^{-4}\Big(\rmi\bar\r^2
		\big((\pd_b\r\s^a\st^b\r)(\pd \bar\r)^\a\pd_a\r_\a
		+ (\pd_a\r\s^a\st^b\pd_b\r)(\r \pd \bar\r) \\\non
	&+\frac12 \r^2 (\r \pd \bar\r)\big)+\cc\Big)
	+|x|^{-6} \r^2\bar\r^2 \left((\pd^a\r \s_{ab}\pd^b\r)
		(\pd^a\bar\r \tilde{\s }_{ab}\pd^b\bar\r)\right) 
									\allowdisplaybreaks\\ %\non
	&-\left(\frac{1}{\sqrt{2}}\bar{\vf }\bar\r 
		+\frac{1}{2}x^{-1}\bar\r^2\bar{\dsF}+\cc\right)\\\non
	&+\frac{1}{4}|x|^{-2}\Big(2(\r\vf )(\bar\r\bar\vf)
		+\r^2\bar\r^2\pd^a\log (x)\pd_a\log (\bar{x})\\\non
	&+\left(2\sqrt{2}\rmi(\r\vf )(\bar\r \pd \r)
		-\r^2(\pd^a\bar\r^2)\pd_a\log(\bar{x})+\cc\right)\Big) 
						\allowdisplaybreaks\\\non
	&+\frac{1}{16}|x|^{-4}\Bigg(\bar\r^2\Big(4\sqrt{2}
		(\r\s^a\bar{\vf})(\pd \bar\r)^\a\pd_a\r_\a 
	+ \sqrt{2}(\pd \bar\r)^\a\pd_{\a\dot\a}(\r^2\bar\vf^\da)\\\non
	&+8\rmi\bar{x}\bar{\dsF}(\r\pd \bar\r)
		+8\rmi(\bar{x}^{-1}\pd_a\bar{x})(\pd^a\r^2)(\r \pd \bar\r)
		+2\sqrt{2}(\pd_b\r\s^a\st^b\r)(\vf \pd_a\r) \\\non
	&+2\sqrt{2}(\pd_a\r\s^a\st^b\pd_b\r)(\vf\r)
		+\sqrt{2}(\square\r^2)(\vf\r)
		+4\rmi(\r\s^a\bar{\vf})(\vf \pd_a\r) \\\non
	&+\rmi\vf^\a\pd_{\a\dot\a}(\r^2\bar{\vf}^{\dot\a}) 
		-4\sqrt{2}\bar{x} \bar{\dsF}(\vf\r )
		-4\sqrt{2}\pd_a\log(\bar{x})(\pd^a\r^2)(\vf\r)\Big)\ +\cc\!\Bigg) 
					\allowdisplaybreaks\\\non
	&+\frac{1}{4}|x|^{-6} \r^2\bar\r^2 \Big(
		-\frac{1}{2}(\bar\vf\pd\r)(\vf\pd\bar\r) + |x \dsF|^2
		+\big\{\rmi\sqrt{2}(\pd^a\r\s_{ab}\pd^b\r)(\vf \pd \bar\r) \\\non
	&+2(\pd^a\r\s_{ab}\pd^b\r)(x \dsF)
		+\frac{\rmi}{\sqrt{2}}(\bar{\vf }\pd\r)(x\dsF) +\cc\! \big\}
		\Big)\Bigg]\,.
\end{align}
In the limit $X\to f$, only the first three lines survive 
and can be checked to match the Samuel-Wess action 
\eqref{mCL:chAV_Action} (or equivalently \eqref{eqn:chAV_Action}).

{\bf TODO: Some discussion? }%TODO


==> A_FeynQuant.tex <==
\chapter[Feynman gauge]{Background field quantization in the Feynman Gauge}
\label{A:FeynQuant}



==> A_GroupTheory.tex <==
\chapter[Group theory]{Group theory for background field loop diagrams}
\label{A:GroupTheory}
Since I've dropped the conformal $\cN=2$ super-Yang-Mills calculations,
I don't really need this section...
%
% Make comments about being careful with group indices because
% do not always use orthonormal basis.


==> Ch_Neq2.tex <==
\chapter{\texorpdfstring{$\cN=2$}{N=2} loop calculations}
\label{Ch:Neq2}
%	N=2 SYM F4
%		Calcs
%		Non-reg probs


==> Extra_CompProj.tex <==
\input{preamble}
%\usepackage{showkeys} 					 %Remove me
\textheight 220mm
\textwidth = 166mm
\evensidemargin -10mm
\oddsidemargin -10mm
\def\baselinestretch{1.2}
\arraycolsep 2pt
\topmargin 0mm
\parskip=\medskipamount

\begin{document}

%TODO Susy current and more robust proof of existence of Goldstinos.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Component projection of a low-energy action} %effective
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Supersymmetric sigma-model}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The most general supersymmetric $\s$-model 
(a maximum of two space-time derivatives) is 
\begin{align}\label{defn:SusySigmaModel}
	S_\s[\Fb,\F] = \intz K(\Fb, \F) + \intc P(\F) + \cc\,,
\end{align}
where $\F^i$ is a multiplet of chiral superfields, $\Db_\da\F^i=0$, 
and $\Fb^\iu$ are antichiral superfields, $D_\a\Fb^\iu=0$.
We define the components of $\F^i$ using
\begin{align}\label{FlatComponentProjPhi}
	\F^i| = \f^i\,,  \qquad
	D_\a\F^i| = \sqrt2 \j^i_\a\,, \qquad
	-\frac14 D^2\F^i| = F^i\,.
\end{align}
Then, the projection of the superpotential is straightforward,
\begin{align}\label{FlatComponentsOfSuperpotential}
	\intc P(\F) &\deq \intx\frac{D^2}{-4}P(\F)\Big|
	=  \intx\frac{D^\a}{-4} D_\a\F^i P_i(\F)\Big| \non \\ \non
	&= \intx\left(\frac{D^2}{-4}\F^i P_i(\F) 
		-\frac{1}{4} D^\a\F^iD_\a\F^j P_{ij}(\F) \right)\Big| \\
	&= \intx\left(F^iP_i(\f) - \frac12 (\j^2)^{ij} P_{ij}(\f)\right)\ .
\end{align}
The component expression for the K\"ahler potential takes a little more work:
\begin{align}\label{FlatComponentsOfKahlerPotential}
	\intz K(\Fb, \F) 
	&\deq \intx\frac{D^\a\Db^2D_\a}{16}K(\Fb, \F)\Big|
	=  \intx\frac{D^\a\Db^2}{16}D_\a\F^i K_{i}(\Fb, \F)\Big| 			\non\\
	&= \intx\frac{D^\a\Db^\da}{16}\left(
		 2\rmi\pd_\ada\F^i K_{i}
		+D_\a\F^i\Db_\da\Fb^\iu K_{i\iu}	\right)\Big|				\non\\
	&= \intx\frac{D^\a}{16}\left(
		 4\rmi\pd_\ada\F^i \Db^\da\Fb^\iu K_{i\iu}
		+D_\a\F^i\Db^2\Fb^\iu K_{i\iu}
		+D_\a\F^i\Db_\da\Fb^\iu\Db^\da\Fb^\ju K_{i\iu\ju} \right)\Big|	\non\\	
%	&= \intx\frac{1}{16}\Big(
%		4\rmi\pd_\ada D^\a\F^i \Db^\da\Fb^\iu K_{i\iu}
%		+8\pd_\ada\F^i \pd^\daa\Fb^\iu K_{i\iu}
%		+4D^\a\F^j\rmi\pd_\ada\F^i \Db^\da\Fb^\iu K_{ij\iu} \non\\
%		&+D^2\F^i\Db^2\Fb^\iu K_{i\iu}
%		-4\rmi D^\a\F^i\pd_\ada\Db^\da\Fb^\iu K_{i\iu}
%		+D^\a\F^j D_\a\F^i\Db^2\Fb^\iu  K_{ij\iu} \non\\
%		&+D^2\F^i\Db_\da\Fb^\iu\Db^\da\Fb^\ju K_{i\iu\ju}
%		-4\rmi D^\a\F^i \pd_\ada\Fb^\iu\Db^\da\Fb^\ju K_{i\iu\ju}
%		+D^\a\F^jD_\a\F^i\Db_\da\Fb^\iu\Db^\da\Fb^\ju K_{ij\iu\ju}
%		 \Big)\Big|	\non\\	
	&= \intx\Big(-\big(
		\pd^a\f^i \pd_a\fb^\iu %-\frac12\pd_\ada\f^i \pd^\daa\fb^\iu 
		+ \frac\rmi2 \j^{i\a}\oLRa{\pd}_\ada\jb^{\iu\da} 
		- F^i\bar{F}^\iu \big) K_{i\iu}	 	\non\\
	&+\frac12\Big(\big(\j^{j\a}(\rmi\pd_\ada\f^i)\jb^{\iu\da} 
		-(\j^2)^{ij}\bar{F}^\iu\big) K_{ij\iu}  + \cc\!\Big)
%	 +\frac12\big(\j^{i\a}(\rmi\pd_\ada\fb^\iu)\jb^{\ju\da}
%		-F^i(\jb^2)^{\iu\ju}\big) K_{i\iu\ju}
	+\frac{1}{4}(\j^2)^{ij}(\jb^2)^{\iu\ju} K_{ij\iu\ju}\Big)\ .
\end{align}

%\begin{align}\label{ComponentSusySigmaModel}
%	S_\s[\Fb,\F] %= \intz K(\Fb, \F) + \intc P(\F) + \cc\,,
%	&= \intx\Big(F^iP_i(\f) + \bar{F}^\iu \bar{P}_\iu(\fb)
%	- \frac12 (\j^2)^{ij} P_{ij}(\f)
%	- \frac12 (\jb^2)^{\iu\ju} \bar{P}_{\iu\ju}(\fb)  \non\\
%	&-\big(\pd^a\f^i \pd_a\fb^\iu 
%		+ \frac\rmi2 \j^{i\a}\oLRa{\pd}_\ada\jb^{\iu\da} 
%		- F^i\bar{F}^\iu \big) K_{i\iu}	 	\\\non
%	&+\frac12\Big(\big(\j^{j\a}(\rmi\pd_\ada\f^i)\jb^{\iu\da} 
%		-(\j^2)^{ij}\bar{F}^\iu\big) K_{ij\iu}  + \cc\!\Big)
%	+\frac{1}{4}(\j^2)^{ij}(\jb^2)^{\iu\ju} K_{ij\iu\ju} \Big)
%\end{align}

In the above, $K_{i\iu}$ is known as the K\"ahler metric. 
It is positive definite if every chiral/scalar field is to have 
a canonical kinetic term $+$ corrections.
The inverse metric is $K^\iui$. 
The nonvanishing Christoffel symbols are 
\begin{align}%\label{}
	\G^i_{jk} = K^{\iui}K_{\iu jk}\,,\qquad
%	\quad\text{and its complex conjugate}\quad
	\G^\iu_{\ju\ku} = K^{\iui}K_{i\ju\ku}\ .
\end{align}
%Later, we will see that this geometric interpretation should be taken seriously,
%and that K\"ahler covariant derivatives and auxiliary fields should be used.

The algebraic equations of motion for the auxiliary fields 
$\bar{F}^\iu$ are
\begin{align}\label{FlatAuxEOM}
	0 = \frac{\d S_\s}{\d {F^i}}
	  =	P_i + \bar{F}^\iu K_{i\iu} - \frac12(\jb^2)^{\iu\ju}K_{i\iu\ju} 
	  \implies
	  \bar{F}^\iu = \frac12\G^\iu_{\ju\ku}(\jb^2)^{\ju\ku}-K^{\iui}P_i\,,
\end{align}
and similarly for its complex conjugate.
%\begin{align*}%\label{}
%	F^i = \frac12\G^i_{jk}(\j^2)^{jk}-K^{\iui}\bar{P}_\iu\ .
%\end{align*}
This can be substituted back into the action to get
the superpotential
\begin{align}\label{ElimSuperpotential}
	\intc P(\F) 
	&= -\intx\left(\bar{P}_\iu K^{\iui}P_i
	- \frac12(\j^2)^{jk}(\G^i_{jk}P_i+P_{jk}) \right)\,,
\end{align}
where clearly the second term is a covariant derivative,
and the K\"ahler potential
\begin{align}\label{ElimKahlerPotential}
	\intz K(\Fb, \F)  
	&= \intx\Big(-\big(
		K_{i\iu} (\pd^a\f^i) (\pd_a\fb^\iu)
		+ \frac\rmi2K_{i\iu} \j^{i\a}\oLRa{\pd}_\ada\jb^{\iu\da} 
		- \bar{P}_\iu K^{\iui}P_i \big) 	 	\\\non
	&+\frac12\Big(\j^{j\a}(\rmi\pd_\ada\f^i)\jb^{\iu\da} K_{ij\iu}
%		+\G^l_{ij}(\j^2)^{ij}P_l -\G^i_{jk}(\j^2)^{jk}P_i
		+ \cc\!\Big) %\non\\
	+\frac14(K_{jk\ju\ku}-\G^i_{jk}K_{i\iu}\G^\iu_{\ju\ku})
		(\j^2)^{jk}(\jb^2)^{\ju\ku}\Big)\ .
\end{align}
The last term contains the Riemann curvature, so it's time to take the
geometric interpretation more seriously.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Covariant representation}\label{ssect:CovRepSigmaModel}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The K\"ahler manifold is parametrized by the complex fields $\f^i$.
A holomorphic change of parametrization is 
$\f^i \to \f'^i = h^i(\f)$. 
This is the lowest component of $\F^i \to \F'^i = h^i(\F)$.
We can then calculate the infinitesimal change in the other components of $\F$.
\begin{align}%\label{}
	\j'^i_\a &= 2^{-1/2}D_\a \F'^i\Big| 
%	= 2^{-1/2}\frac{\pd\F'^i}{\pd\F^j} D_\a \F^j\Big|
	= \frac{\pd\f'^i}{\pd\f^j} \j^j_\a\,, \\
	F'^i &= \frac{D^2}{-4}\F'^i\Big|
%	=  \frac{D^\a}{-4}\frac{\pd\F'^i}{\pd\F^j} D_\a \F^j\Big|
%	= \frac{\pd\F'^i}{\pd\F^j}  \frac{D^2}{-4} \F^j
%	- \frac{1}{4}\frac{\pd^2\F'^i}{\pd\F^j\pd\F^k}D^\a\F^k D_\a \F^j\Big|
	=  \frac{\pd\f'^i}{\pd\f^j} F^j 
	- \frac12 \frac{\pd^2\f'^i}{\pd\f^j\pd\f^k} (\j^2)^{jk}\,,
\end{align}
so the $\j^i_\a$ transforms as a vector, 
but $F^i$ transforms inhomogeneously, we will fix this momentarily.
First, we note that the action is invariant if
\begin{align*}%\label{}
	K'(\Fb',\F') = K(\Fb, \F)
	\quad \text{and} \quad P'(\F')=P(\F)\,,
\end{align*}
which means that $K_i$ and $P_i$ (and complex conjugates) transform as covectors 
and the K\"ahler metric transforms covariantly
\begin{align}%\label{}
	K'_{,i\iu}(\Fb,\F) 
	= \frac{\pd\F^j}{\pd\F'^i}\frac{\pd\Fb^\ju}{\pd\Fb'^\iu}K_{,j\ju}(\Fb,\F)
	\implies
	K'_{i\iu} =\frac{\pd\f^j}{\pd\f'^i}\frac{\pd\fb^\ju}{\pd\fb'^\iu}K_{j\ju}\ .
\end{align}
We can then calculate the transformation of the Christoffel symbols as
\begin{align}%\label{}
	\G'^i_{jk} = K'^{\iui}K'_{jk\iu}
	= \frac{\pd\f^n}{\pd\f'^k}\frac{\pd\f^m}{\pd\f'^j}
		\frac{\pd\f'^i}{\pd\f^l}\G^l_{mn}
	+ \frac{\pd^2\f^m}{\pd\f'^j\pd\f'^k}\frac{\pd\f'^i}{\pd\f^m}\ .
\end{align}
Now we can define a covariantly transforming auxiliary field
\begin{align}\label{defn:KahlerCovAuxField}
	F_\text{cov}^i = F^i - \frac12 \G^i_{jk}(\j^2)^{jk} 
	\implies
	F'^i_\text{cov} = \frac{\pd\f'^i}{\pd\f^j}F^j_\text{cov}\ .
\end{align}
%Check the covariant transformation:
%\begin{align*}
%	F'^i_\text{cov} &= F'^i - \frac12 \G'^i_{jk}(\j'^2)^{jk} \\
%	&=\frac{\pd\f'^i}{\pd\f^j} F^j 
%	- \frac12 \frac{\pd^2\f'^i}{\pd\f^j\pd\f^k} (\j^2)^{jk} 
%	- \frac12 (\frac{\pd\f^n}{\pd\f'^k}\frac{\pd\f^m}{\pd\f'^j}
%		\frac{\pd\f'^i}{\pd\f^l}\G^l_{mn}
%	+ \frac{\pd^2\f^m}{\pd\f'^j\pd\f'^k}\frac{\pd\f'^i}{\pd\f^m})
%	\frac{\pd\f'^j}{\pd\f^p}\frac{\pd\f'^k}{\pd\f^q}(\j^2)^{pq}\\
%	&=\frac{\pd\f'^i}{\pd\f^j} F^j 
%	- \frac12 \frac{\pd^2\f'^i}{\pd\f^j\pd\f^k} (\j^2)^{jk} 
%	- \frac12 \frac{\pd\f'^i}{\pd\f^l}\G^l_{jk}(\j^2)^{jk}
%	- \frac12 (\frac{\pd}{\pd\f'^j}\frac{\pd\f^m}{\pd\f'^k})
%	\frac{\pd\f'^i}{\pd\f^m}\frac{\pd\f'^j}{\pd\f^p}\frac{\pd\f'^k}{\pd\f^q}
%	(\j^2)^{pq}\\
%	&=\frac{\pd\f'^i}{\pd\f^j} \Big(F^j 
%	- \frac12 \G^j_{kl}(\j^2)^{kl}\Big)
%	- \frac12 \frac{\pd^2\f'^i}{\pd\f^j\pd\f^k} (\j^2)^{jk} 
%	- \frac12 (\frac{\pd}{\pd\f^p}\frac{\pd\f^m}{\pd\f'^k})
%	\frac{\pd\f'^i}{\pd\f^m}\frac{\pd\f'^k}{\pd\f^q}(\j^2)^{pq} \\
%	&=\frac{\pd\f'^i}{\pd\f^j} \Big(F^j 
%	- \frac12 \G^j_{kl}(\j^2)^{kl}\Big)
%	- \frac12 \frac{\pd^2\f'^i}{\pd\f^j\pd\f^k} (\j^2)^{jk} 
%	- \frac12 \Big(\frac{\pd}{\pd\f^p}(\frac{\pd\f^m}{\pd\f'^k}
%		\frac{\pd\f'^i}{\pd\f^m}) 
%		- \frac{\pd\f^m}{\pd\f'^k}\frac{\pd^2\f'^i}{\pd\f^p\pd\f^m}\Big)
%	\frac{\pd\f'^k}{\pd\f^q}(\j^2)^{pq}\\
%	&=\frac{\pd\f'^i}{\pd\f^j} \Big(F^j 
%	- \frac12 \G^j_{kl}(\j^2)^{kl}\Big)
%	- \frac12 \frac{\pd^2\f'^i}{\pd\f^j\pd\f^k} (\j^2)^{jk} 
%	- \frac12 \Big(0 - \frac{\pd^2\f'^i}{\pd\f^p\pd\f^q}\Big)(\j^2)^{pq}
%	= \frac{\pd\f'^i}{\pd\f^j} F^j_\text{cov} .
%\end{align*}
Now we introduce the K\"ahler covariant derivatives
\begin{align}\label{TargetSpaceCovDeriv}
	\nabla_j V^i = V^i_{;j} = V^i_{,j} + \G^i_{jk}V^k \,,\quad
	\nabla_j V_i = V_{i;j} = V_{i,j} - \G^k_{ij}V_k \,,
\end{align}
and the target space covariant derivatives
\begin{align}\label{SpaceTimeTargetSpaceCovDeriv}
	\nabla_a\j^i_\a = \pd_a\j^i_\a + \G^i_{jk}(\pd_a\f^j)\j^k_\a \,,\quad
	\nabla_a\jb^\iu_\da = \pd_a\jb^\iu_\da 
		+ \G^\iu_{\ju\ku}(\pd_a\fb^\ju)\jb^\ku_\da \ .
\end{align}
Finally, note that the only non-vanishing Riemann tensor components are
\begin{align}%\label{}
	\cR_{i\ju k\lu} = K_{i\iu j\ju} - K^{\ku k}K_{ij\ku}K_{k\iu\ju}
	= K_{i\iu j\ju} - \G^k_{ij}K_{k\ku}\G^\ku_{\iu\ju}\ .
\end{align}

Now we can write the uneliminated component result using the above
covariant quantities,
\begin{align}\label{CovComponentSusySigmaModel}
	\cL_\s 
	&= \big(F_\text{cov}^iP_i 
	- \frac12 (\j^2)^{ij} P_{;ij} + \cc \big)\non\\
	&-K_{i\iu}\big(\pd^a\f^i \pd_a\fb^\iu 
		+ \frac\rmi2 \j^{i\a}\oLRa{\nabla}_\ada\jb^{\iu\da} 
		- F_\text{cov}^i\bar{F}_\text{cov}^\iu  \big) 	
		+\frac{1}{4}(\j^2)^{ij}(\jb^2)^{\iu\ju} \cR_{ij\iu\ju} \ .
\end{align}
The covariant auxiliary fields' equations are simply 
$P_i = K_{i\iu}\bar{F}_\text{cov}^\iu$, 
so the eliminated component Lagrangian is
\begin{align}\label{CovEliminatedSusySigmaModel}
	\cL_\s 
	&= -\pd_a\fb^\iu K_{i\iu} \pd^a\f^i  
	- \frac\rmi2 K_{i\iu} \j^{i\a}\oLRa{\nabla}_\ada\jb^{\iu\da} 
	- \bar{P}_\iu K^{\iui} P_i 	\non\\
	&- \frac12(\j^2)^{ij} P_{;ij} - \frac12(\jb^2)^{\iu\ju} \bar{P}_{;\iu\ju}
	+\frac{1}{4}(\j^2)^{ij}(\jb^2)^{\iu\ju} \cR_{ij\iu\ju} \ .
\end{align}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Supersymmetry breaking}\label{ssect:SusyBreakingSigmaModel}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The vacuum state $\ket\vac$ does not break supersymmetry iff it is invariant
under all of the supersymmetry generators
\begin{align}\label{SusyInvarianceOfVac}
	Q_\a\ket\vac = \bar{Q}_\da\ket\vac = 0\ .
\end{align}
From the supersymmetry algebra, this implies that the vacuum must
also be invariant \wrt the energy-momentum generators. 
In particular, this implies that the energy of the vacuum is nonnegative
\begin{align}\label{NonNegativeSusyVacuum}
	\VEV{H} &= \VEV{P_0} %= -\frac14\VEV{\st_0^{\ada}\acom{Q_\a}{\bar{Q}_\da}}
	= \frac14\VEV{\d^{\ada}\acom{Q_\a}{\bar{Q}_\da}} \non\\
	&= \frac14\big(\big\|Q_1\ket\vac\!\big\|^2 + \big\|Q_2\ket\vac\!\big\|^2
		+ \big\|\bar{Q}_1\ket\vac\!\big\|^2 
		+ \big\|\bar{Q}_2\ket\vac\!\big\|^2 \big)\ .
\end{align}
So the vacuum energy can be thought of as an order parameter for susy breaking.

In a Lorentz invariant vacuum, 
only the scalar fields can have a non zero value, 
or vacuum expectation value (VEV):
\begin{align*}%\label{}
	\VEV{\l^i_\a} = \VEV{\pd_a\f^i} = 0\ .
\end{align*}
Equation \eqref{SusyInvarianceOfVac} also implies that 
supersymmetry is preserved by the vacuum if the vacuum expectation value 
of all susy variations is zero. %Given the component supersymmetry transformations,
The variation of bosonic fields is always fermionic, which must vanish due
to Lorentz invariance, 
so all that matters is the variation of the spinor fields.
\begin{align*}%\label{}
	\VEV{\d_{\x}\l_\a} 
	= \sqrt{2}\big(\x_\a \VEV{F} + \rmi(\s^a\bar\x)_\a\VEV{\pd_a\f}\big)\ .
\end{align*}
the last term must vanish in a Lorentz invariant vacuum, 
so supersymmetry is preserved iff the auxiliary field has 
no vacuum expectation value.


Now let's specialize to the K\"ahler models studied above.
In this case,  the vacuum energy can also be seen to be nonnegative
from the scalar potential of \eqref{CovEliminatedSusySigmaModel}
\begin{align}
	V = \bar{P}_\iu K^{\iui} P_i \geq 0\ .
\end{align}
It is positive semi-definite, since we required 
that the scalar fields have canonical kinetic terms 
(so $K_{i\iu} = \d_{i\iu} + \text{higher order terms}$).
Supersymmetry is preserved iff the VEV of the scalar potential is zero,
and since the K\"ahler metric is positive semi-definite, this implies that
supersymmetry is preserved iff there is a solution to the simultaneous equations
\begin{align}%\label{}
	P_i(\expt\f) = \bar{P}_\iu(\expt\fb) = 0 \ .
\end{align}
Note that if such a solution exists, then it is 
automatically a minimum of the potential, so a possible vacuum.
Since $P_i = K_{i\iu}\bar{F}_\text{cov}^\iu$ 
and $\expt{F^i_\text{cov}}=\expt{F^i}$, 
we see once again that supersymmetry is broken
only if there is a nonvanishing VEV for one or more of the auxiliary fields 
$F^i$. This is known as $F$-term SUSY breaking.
 
In general, a (false or true) vacuum 
is at a (local or global) minimum of the scalar potential.
Noting that 
\( K^{\iui}_{,j} = -K^{\iu k}\G^i_{kj} \)
gives us a covariant form for the first derivative of the scalar potential
\begin{align}\label{CovFirstDerivOfV}
 V_j = \bar{P}_\iu K^{\iui} P_{i,j} -  \bar{P}_\iu K^{\iu k}\G^i_{kj} P_i
	= \bar{P}_\iu K^{\iui} P_{;ij}\ .
\end{align}
If supersymmetry is not broken, then $\bar{P}_\iu=0$ and we are automatically
at a minimum of the potential.
If supersymmetry is broken, it tells us that 
the nonvanishing vector $\bar{P}_\iu K^{\iui}$ is a null vector for $P_{;ij}$. 
%i.e.\ $P_i(\f) \neq 0 \neq \bar{P}_\iu$ and $\bar{P}_\iu K^{\iui} P_{;ij}=0$

Now note that the fermion mass term is proportional to $\j^{i\a}P_{;ij}\j^j_\a$.
%NB $P_{;ij}=P_{;ji}$.
Assuming that the vacuum breaks supersymmetry, equation \eqref{CovFirstDerivOfV}
implies that the fermion mass matrix has the null vector $\VEV{F^i}$
and so there must exist a massless fermion, the Goldstino.
If we think about an changing the fermion basis to one that includes
the null vector,
%\[ \l B B^T P B B^T \l ,  
% B = (.... , <F>/\sqrt{<F K Fb>}),  B^T = <K Fb>/\sqrt{<F K Fb>} \]
then we see that the Goldstino is proportional to
\begin{align*}%\label{}
	G_\a \propto \l^i_\a \VEV{K_{i\iu} \bar{F}^\iu}\ .
\end{align*}
%Only the variation of the fermions can have a nonvanishing expectation value.



The simplest model with $F$-term supersymmetry breaking has only one superfield
\begin{align*}%\label{}
	S[\Fb,\F] = \intz\Fb\F + \intc f\F + \intac \bar{f}\Fb\,,
\end{align*}
and the constant $f$ can be chosen to be real.
In this case, the derivative of the superpotential is $\pd_\F P(\F) = f$
which is non-zero, so by the above criteria, supersymmetry is broken.
The component Lagrangian is
\begin{align*}%\label{}
	\cL = - \pd^a\fb\pd_a\f -\frac12\l\oLRa{\pd}\bar\l 
		+ \bar{F}F + f F + \bar{f}\bar{F}
		= -\bar{f}f - \pd^a\fb\pd_a\f -\frac12\l\oLRa{\pd}\bar\l  \,,
\end{align*}
where the second equality follows from putting the auxiliary fields on-shell.
Clearly this describes a free theory with broken supersymmetry and a 
vacuum energy density of $|f|^2$. 
Both the goldstino $\l_\a$ and its superpartner $\f$ are massless.
Although this model is trivial, if the chiral field is constrained,
then we can obtain non-trivial Goldstino dynamics equivalent to that of
Akulov and Volkov. This will be investigated further in the following chapters.

The simplest interacting model of chiral superfields 
that breaks supersymmetry was found by O'Raifeartaigh \cite{O'Raifeartaigh1975}. 
It requires three chiral superfields, with the canonical K\"ahler potential
and the superpotential
\begin{align*}%\label{}
	P(\F^i) = m\F_1\F_2 + g\F_0(\F_1^2-\a^2)\,,
\end{align*}
where again, the coupling constants can be chosen, 
without loss of generality, to be real.
For non-zero $g\a^2$, the equations 
$P_{,0} = g(\f_1^2-\a^2) = 0 = m\f_1 = P_{,2}$ are not compatible, 
so supersymmetry is broken.
The scalar potential is
\begin{align*}%\label{}
	V = |g|^2|\f_1^2-\a^2|^2 + |m\f_1|^2 + |m\f_2+2g\f_0\f_1|^2\ .
\end{align*}
Minimizing the first two terms fixes $\f_1$ and the final term can 
be made zero by the appropriate choice of $\f_2$. 
This means the minimum of potential has a flat direction along $\f_0$.
The fermion mass matrix 
\[ P_{ij} = \bem0&2g\f_1&0\\2g\f_1&g\f_0&m\\0&m&0\eem\,, \]
has a vanishing determinant (for $m\neq0$, it has a null space of dimension 1), 
establishing the existence of the massless Goldstino.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{A gauged sigma-model}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
If the sigma model has global isometries, 
they can be gauged (made local) by adding suitable gauge fields. 
We will assume that this is the case and start off with 
the most general non-renormalizable low-energy action 
of interacting chiral and real (gauge) superfields,
\begin{align}\label{defn:GaugedSusySigmaModel}
	S_\s[\Fb,\F,\cW,\cWb] 
	= S_\s[\Fb,\F]
		+ \Big(\frac14\intc f_{\m\n}(\F)\cW^{\m\a}\cW^\n_\a + \cc\Big)
		+ \intz \k_\m V^\m\,,
%	= \intz K(\Fb, \F)
%	+ \intc\big(P(\F)+f_{\m\n}(\F)\cW^{\m\a}\cW^\n_\a \big) + \cc\,,
\end{align}
where $S_\s[\Fb,\F]$ is as in \eqref{defn:SusySigmaModel}
but now $\F^i$ is a multiplet of \emph{gauge covariantly} chiral superfields, 
$\cDb_\da\F^i=\cD_\a\Fb^\iu=0$.
The second term is the effective gauge kinetic term, 
which is constructed from the field strength superfields\footnote%
{See the quantization of $\cN=1$ SYM chapter for more information.}
$T_\m\cW_\a^\m=-\frac18\cDb^2\rme^{-V}\cD_\a\rme^V$ 
%for some reductive (if it's to be quantized) Lie algebra
and the gauge kinetic function, $f_{\m\n}(\F)$, 
which at leading order is like $\d_{\m\n}/g^2$ 
and $g^2$ can vary for each connected component of the Lie algebra.\footnote%
{Note that this is \emph{not} the most general case as the isometry group 
of the scalar manifold does not have to be a compact Lie group, 
in which case the Killing vectors will be more general than 
$\x_\m^i(\f)=(\rmi T_\m \f)^i$.}
%$f_{\m\n}(\F) \approx \frac{T(\cR)^{-1}}{g^2_{(\cR)}}g_{\m\n}^{(\cR)} + O(\F)$
The final term is the Fayet-Iliopoulos term and if it is to be gauge invariant, 
the coefficient $\k_a$ most only be non-vanishing for 
abelian factors of the Lie group.

The gauge covariant component projections of the chiral fields are 
exactly as in \eqref{FlatComponentProjPhi}, but with $D_\a\to\cD_\a$.
We define the %gauge covariant 
components of the gauge field strength as\footnote%
{Note that we will use $\cF_{ab}$ both for the superfield 
and its lowest component. This should be clear from context.
Similarly, $\cD_{\ada}=\s_\ada^a\cD_a$ will mean the gauge covariant derivative
at both the superfield and component field level. 
In this chapter, we reserve $\nabla$ for the target space covariant derivatives.
}
\begin{align}\label{FieldStrengthComponentProj}
	\cW_\a^\mu| = \l_\a^\m\,,  \qquad
	\cD_{(\a}\cW_{\b)}^\mu| = 2\rmi \cF_{\a\b}^\mu 
		= \rmi(\s^{ab})_{\a\b}\,\cF^\m_{ab}\,, \qquad
	\cD^\a\cW_\a^\mu| = -2D^\mu\ .
\end{align}%See eq 1.2.33 of B&K for conventions on field strength-type tensors.
Combined with the covariant $\cD$-algebra, this implies that
\begin{align*}%\label{}
	\cD_\b \cW_\a &= \cD_{(\a}\cW_{\b)} -\frac12\eps_{\a\b} \cD^\g\cW_\g\,,&
	\cD^2\cW_\a &= 4\rmi\cD_\ada \cWb^\da\ .
\end{align*}

Now we can examine the component projections.
%
The simplest term is the Fayet-Iliopoulos term -- a pure $D$ term,
\begin{align}\label{FI-term-ComponentProj}
	S_\text{FI} = \intz \k_\m V^\m 
%	= \frac1{16}\intx\k_\m D^\a \Db^2 D_\a V^\m
	= -\frac1{2}\intx\k_\m D^\a W_\a^\m
	= \intx\k_\m D^\m\ .
\end{align}
%
The component form of the superpotential does not change from the non-gauge case
\eqref{FlatComponentsOfSuperpotential}, 
except that now the components are gauge covariant.
\begin{align}%\label{FlatComponentsOfSuperpotential}
	\intc P(\F) %&\deq \intx\frac{D^2}{-4}P(\F)\Big|
	= \intx\left(F^iP_i(\f) - \frac12 (\j^2)^{ij} P_{ij}(\f)\right)\ .
\end{align}
%
The gauge kinetic term, being chiral, is also quite simple:
\begin{align}\label{GaugeKineticComponentProj}
	\intc f_{\m\n}(\F)(\cW^2)^{\m\n}
%	&= \intx\Big( \frac12 f_{\m\n}(\F) 
%		\big(\cD^\b\cW^{\m\a}\cD_\b\cW^\n_\a
%		-\cW^{\m\a}\cD^2\cW^\n_\a\big) \non\\
%	&+\cD^\b\F^i f_{\m\n,i}(\F)\cW^{\m\a}\cD_\b\cW^\n_\a
%	-\frac14\big(\cD^2\F^i f_{\m\n,i}(\F)
%	+\cD^\b\F^i\cD_\b\F^j f_{\m\n,ij}(\F)\big) \cW^{\m\a}\cW^\n_\a \Big)\Big| 
%	\non\\
%	&= \intx\Big( \frac12 f_{\m\n}(\F) 
%		\big(\frac12(\cD\cW)^\m(\cD\cW)^\n - 4\rmi\cW^{\m\a}\cD_\ada\cWb^{\n\da}
%		-\cF^\m_{ab}\cF^{\n ab}-\cF^\m_{ab}\tilde\cF^{\n ab}\big) \non\\
%	&+\cD^\b\F^i f_{\m\n,i}(\F)\cW^{\m\a}
%		\big(\cD_{(\b}\cW^\n_{\a)}-\frac12\eps_{\a\b}(\cD\cW)^\n\big) \non\\
%	&-\frac14\big(\cD^2\F^i f_{\m\n,i}(\F)
%	+\cD^\b\F^i\cD_\b\F^j f_{\m\n,ij}(\F)\big) \cW^{\m\a}\cW^\n_\a \Big) \Big|
%	\non \\
	&= \intx\Big( f_{\m\n} 
		\big( D^\m D^\n - 2\rmi\l^{\m\a}{\cD}_\ada\bar\l^{\n\da}
		-\frac12\cF^\m_{ab}\cF^{\n ab}
		-\frac12 \cF^\m_{ab}\tilde\cF^{\n ab}\big) \\\non
	&+\sqrt2\j^{i\b} f_{\m\n,i} \l^{\m\a}
		\big(2\rmi\cF^\n_{\a\b}+\eps_{\a\b}D^\n\big) 
	+ \big(F^i f_{\m\n,i} 
	- \frac12(\j^2)^{ij} f_{\m\n,ij} \big)(\l^2)^{\m\n} 	\Big)\,,
\end{align}
where the dual field strength is defined as 
$\tilde\cF^{ab}=\frac\rmi2\eps^{abcd}\cF_{cd}$.
The K\"ahler potential is similar to \eqref{FlatComponentsOfKahlerPotential}, 
except extra contributions come from the gauge covariant $\cD$-algebra:
{\allowdisplaybreaks
\begin{align}\label{GaugeComponentsOfKahlerPotential}
	\intz K(\Fb, \F) %	&\deq \intx\frac{D^\a\Db^2D_\a}{16}K(\Fb, \F)\Big|
&= \intx\frac{\cD^\a\cDb^2}{16}\cD_\a\F^i K_{i}(\Fb, \F)\Big| 			\non\\
%&= \intx\frac{\cD^\a}{16}\Big(	\cDb^2\cD_\a\F^i K_{i} 
%		- 2\cDb_\da\cD_\a\F^i\cDb^\da\Fb^\iu K_{i\iu}
%		+ \cD_\a\F^i \cDb^2 K_{i} \Big)\Big|	 \non\\
%&= \intx\frac{\cD^\a}{16}\Big(	-8(\cW_\a\F)^i K_{i} 
%		+ 4\rmi\cD_\ada\F^i\cDb^\da\Fb^\iu K_{i\iu} \non\\
%	&+ \cD_\a\F^i \cDb^2\Fb^\iu K_{i\iu}
%	 + \cD_\a\F^i \cDb_\da\Fb^\ju \cDb^\da\Fb^\iu K_{i\iu\ju} \Big)\Big| \non\\
%&= \intx\frac{1}{16}\Big(	-8(\cD^\a\cW_\a\F)^i K_{i} 
%		-8(\cW^\a\cD_\a\F)^i K_{i} - 8\cD^\a\F^j(\cW_\a\F)^i K_{ij} \non\\
%	&+ 4\rmi\cD_\ada\cD^\a\F^i\cDb^\da\Fb^\iu K_{i\iu}
%	 - 16(\cWb_\da\F)^i\cDb^\da\Fb^\iu K_{i\iu}
%	 + 8\cD_\ada\F^i\cD^\ada\Fb^\iu K_{i\iu}
%	 - 4\rmi\cD_\ada\F^i\cDb^\da\Fb^\iu \cD^\a\F^j K_{ij\iu} \non\\
%	&+ \cD^2\F^i \cDb^2\Fb^\iu K_{i\iu}
%	- 4\rmi\cD_\a\F^i \cD^\ada\cDb_\da\Fb^\iu K_{i\iu}
%	- 8\cD_\a\F^i (\cW^\a\Fb)^\iu K_{i\iu}
%	+ \cD^\a\F^j\cD_\a\F^i \cDb^2\Fb^\iu K_{ij\iu} \non\\
%	&+ \cD^2\F^i \cDb_\da\Fb^\ju \cDb^\da\Fb^\iu K_{i\iu\ju} 
%	- 4\rmi \cD_\a\F^i \cDb_\da\Fb^\ju \cD^\ada\Fb^\iu K_{i\iu\ju}
%	+ \cD^\a\F^j\cD_\a\F^i \cDb_\da\Fb^\ju \cDb^\da\Fb^\iu K_{ij\iu\ju}
%	\Big)\Big| \non\\
%&= \intx\Big( (D\F)^i K_{i} - 2^{-1/2}(\l^\a\j_\a)^i K_{i} 
%	 - 2^{-1/2}\j^{j\a}(\l_\a\f)^i K_{ij} \non\\
%	&+ \frac\rmi2\cD_\ada\j^{i\a}\jb^{\iu\da} K_{i\iu}
%	 - \sqrt{2}(\bar\l_\da\f)^i\jb^{\iu\da} K_{i\iu}
%	 + \frac12\cD_\ada\f^i\cD^\ada\fb^\iu K_{i\iu}
%	 + \frac\rmi2\j^{i\a}\cD_\ada\f^j\bar\j^{\iu\da} K_{ij\iu} \non\\
%	&+  F^i \bar{F}^\iu K_{i\iu}
%	- \frac\rmi2\j^{i\a} \cD_\ada \jb^{\iu\da} K_{i\iu}
%	- 2^{-1/2}\j^{i}_{\a} (\l^\a\fb)^\iu K_{i\iu}
%	- \frac12\j^{j\a}\j^i_{\a} \bar{F}^\iu K_{ij\iu} \non\\
%	&- \frac12 F^i \jb^\ju_{\da} \jb^{\iu\da} K_{i\iu\ju} 
%	- \frac\rmi2 \j_\a^i \jb_\da^\ju \cD^\ada\fb^\iu K_{i\iu\ju}
%	+ \frac14(\j^2)^{ij} (\jb^2)^{\iu\ju} K_{ij\iu\ju}	\Big) \non\\
&= \intx\Big( (D\f)^i K_{i} - 2^{-1/2}(\l^\a\j_\a)^i K_{i} 
	 - 2^{-1/2}(\l^\a\f)^i\j^{j}_{\a} K_{ij} \non\\
	 &- \sqrt{2}(\bar\l_\da\f)^i\jb^{\iu\da} K_{i\iu}
	 %TODO The following - sign is a fudge! Fix it!!
	 - 2^{-1/2} (\l^\a\fb)^\iu \j^{i}_{\a} K_{i\iu} \non\\
	&- \Big( \frac\rmi2\j^i_{\a} \oLRa{\cD}{}^\ada\jb^\iu_{\da} %K_{i\iu}
	 + \cD_a\f^i\cD^a\fb^\iu %K_{i\iu}
	 -  F^i \bar{F}^\iu \Big) K_{i\iu} \\\non 
	&+ \Big\{\Big(\frac\rmi2\j^{i\a}\cD_\ada\f^j\bar\j^{\iu\da} %K_{ij\iu} 
	- \frac12(\j^2)^{ij} \bar{F}^\iu \Big)K_{ij\iu} + \cc\Big\} 
	+ \frac14(\j^2)^{ij} (\jb^2)^{\iu\ju} K_{ij\iu\ju}
	\Big) \ . %\non\\
\end{align}}

The first two lines of the final equality 
in \eqref{GaugeComponentsOfKahlerPotential} 
contain the component fields of the gauge multiplet and are not explicitly real. 
Of course, the gauging of the susy $\s$-model is only possible 
if the K\"ahler potential and superpontential are gauge invariant,\footnote%
{Only the action \eqref{defn:GaugedSusySigmaModel}
actually needs to be invariant, 
so both terms only need to be invariant up to total derivative,
and the K\"ahler potential can be invariant up to K\"ahler transformations.}
and it is exactly the former of these properties we need 
to show the reality of \eqref{GaugeComponentsOfKahlerPotential}:
\begin{align}\label{ConsqOfGaugeInvKahler}
\begin{aligned}
	&K(\Fb\rme^{-\rmi\k},\rme^{\rmi\k}\F) = K(\Fb,\Fb)
	\implies (T_\m\F)^i K_i = (\Fb T_\m)^\iu K_\iu \\
	\implies 
	&(D\f)^i K_i = (\fb D)^\iu K_\iu
	\quad\text{and}\quad
	(\l^\a\j_\a)^i K_{i} + (\l^\a\f)^i \j^j_{\a} K_{ij} 
	= (\l^\a\fb)^\iu \j^{i}_{\a} K_{i\iu}\ .
\end{aligned}
\end{align}
So we can write the component expression for the K\"ahler potential as
\begin{align}\label{GaugeComponentsOfKahlerPotential2}
	\intz K(\Fb, \F)
&=\intx\Big( \frac12\big((D\f)^i K_{i} + \cc) 
%	 - \sqrt{2}(\bar\l_\da\f)^i\jb^{\iu\da} K_{i\iu}
	 - \sqrt{2} \big((\l^\a\fb)^\iu \j^{i}_{\a} +\cc\big) K_{i\iu} \non\\
	&- \Big( \frac\rmi2\j^i_{\a} \oLRa{\cD}{}^\ada\jb^\iu_{\da} %K_{i\iu}
	 + \cD_a\f^i\cD^a\fb^\iu %K_{i\iu}
	 -  F^i \bar{F}^\iu \Big) K_{i\iu} \\\non 
	&+ \Big\{\Big(\frac\rmi2\j^{i\a}\cD_\ada\f^j\bar\j^{\iu\da} %K_{ij\iu} 
	- \frac12(\j^2)^{ij} \bar{F}^\iu \Big)K_{ij\iu} + \cc\Big\} 
	+ \frac14(\j^2)^{ij} (\jb^2)^{\iu\ju} K_{ij\iu\ju}
	\Big) \ .
\end{align}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Covariant representation}\label{ssect:CovRepGaugedSigmaModel}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Now we rewrite the above action using the covariant objects of 
subsection \ref{ssect:CovRepSigmaModel}, except that now the component fields 
are gauge covariant and the target space covariant space-time derivative of
\eqref{SpaceTimeTargetSpaceCovDeriv} uses gauge covariant derivatives
instead of normal partial derivatives, i.e., $\pd_a\to\cD_a$.
%
The Fayet-Iliopoulos term remains unchanged. 
\begin{align*}\tag{\ref{FI-term-ComponentProj}}
	S_\text{FI} = \intz \k_\m V^\m 
%	= \frac1{16}\intx\k_\m D^\a \Db^2 D_\a V^\m
%	= -\frac1{2}\intx\k_\m D^\a W_\a^\m
	= \intx\k_\m D^\m\ .
\end{align*}
The covariant form of the effective potential is functionally 
the same as the non-gauge case 
\begin{align}%\label{CovComponentsOfSuperpotential}
	\intc P(\F) %&\deq \intx\frac{D^2}{-4}P(\F)\Big|
	= \intx\left(F_\text{cov}^iP_i(\f) 
		- \frac12 (\j^2)^{ij} P_{;ij}(\f)\right)\,,
\end{align}
which is the same as the covariantization of the gauge kinetic action, 
as it only effects the final term
\begin{align}\label{CovGaugeKineticComponentProj}
	\intc f_{\m\n}(\F)(\cW^2)^{\m\n}
	&= \intx\Big( f_{\m\n} 
		\big( D^\m D^\n - \rmi(\l^{\m}\oLRa{\cD}\bar\l^{\n})
		-\frac12(\cF^2)^{\m\n} -\frac12 (\cF\tilde\cF)^{\m\n}\big)  \\\non
	&+\sqrt2\j^{i\b} f_{\m\n,i} \l^{\m\a}
		\big(2\rmi\cF^\n_{\a\b}+\eps_{\a\b}D^\n\big) 
	+ \big(F_\text{cov}^i f_{\m\n,i} 
	- \frac12(\j^2)^{ij} f_{\m\n;ij} \big)(\l^2)^{\m\n} 	\Big)\ .
\end{align}
Finally, the covariantization of the K\"ahler potential is
also functionally the same as the non-gauge case
\begin{align}\label{GaugeComponentsOfKahlerPotential-Cov}
	\intz K(\Fb, \F)
&=\intx\Big( \frac12\big((D\f)^i K_{i} + \cc) 
	 - \sqrt{2} \big((\l^\a\fb)^\iu \j^{i}_{\a} +\cc\big) K_{i\iu} \non\\
	&- \Big( \frac\rmi2\j^i_{\a} \oLRa{\nabla}{}^\ada\jb^\iu_{\da} %K_{i\iu}
	 + \cD_a\f^i\cD^a\fb^\iu %K_{i\iu}
	 -  F_\text{cov}^i \bar{F}_\text{cov}^\iu \Big) K_{i\iu} 
	 + \frac14(\j^2)^{ij} (\jb^2)^{\iu\ju} \cR_{ij\iu\ju}
	\Big) \ .
\end{align}

The equations of motion for the auxiliary fields are 
\begin{align}%\label{}
	0 &= \frac{\d S}{\d D^\m}
	= \k_\m + \hat{f}_{\m\n}D^\n 
		- \frac1{2\sqrt{2}}\big(\j^{i\a}f_{\m\n,i}\l^\n_\a+\cc\big)
		+ \frac12\big((T_\m\f)^i K_i + \cc\big)\,, \\
	0 &= \frac{\d S}{\d F_\text{cov}^i}
	= P_i + \frac14 f_{\m\n,i}(\l^2)^{\m\n} + \bar{F}_\text{cov}^\iu K_{i\iu}\,,
	\quad\text{and}\quad\cc\!,
\end{align}
where $\hat{f}_{\m\n}=\frac12({f}_{\m\n}+\bar{f}_{\m\n})$.
These are algebraic equations, so can be simply solved for $D^\m$ and 
$F_\text{cov}^i$ then substituted back into the action
to get the eliminated action.
%\begin{align*}%\label{}
%	\cL = 
%\end{align*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Supersymmetry breaking}\label{ssect:SusyBreakingGaugedSigmaModel}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
All the arguments at the top of subsection \ref{ssect:SusyBreakingSigmaModel}
are still relevant for the gauged case. 
So, both the vacuum energy and auxiliary field VEVs 
are order parameters for susy breaking.
However, now there are two types of auxiliary fields, 
$F\sim F_\text{cov}$ and $D$. 
Susy breaking can be of either $F$-type, $D$-type or mixed.

The vacuum potential is found from the Lagrangian by setting all derivatives
and fermion and vector fields to zero (and multiplying by $-1$)
\begin{align*}%\label{}
	-V &= \k_\m D^\m + \frac12 D^\m \hat{f}_{\m\n} D^\n 
	+ \frac12\big((D\f)^i K_i + \cc) 
	+ (F_\text{cov}^i P_i + \cc)
	+ F_\text{cov}^i K_{i\iu} \bar{F}_\text{cov}^\iu \ .
\end{align*}
Define $X_\m = \frac12\big((T_\m\f)^i K_i + \cc)$, then 
the auxiliary field equations of motion in the effective potential approximation 
are $D^\m = -\hat{f}^{\m\n}(\k_\n+X_\n)$ 
and $\bar{F}_\text{cov}^\iu=-K^{\iu i}P_i$.
So we can eliminate the auxiliary fields to get the scalar potential
\begin{align*}%\label{}
	V%_\text{elim} 
	&= \frac12 (\k_\m + X_\m)\hat{f}^{\m\n}(\k_\n + X_\n)
		+ \bar{P}_\iu K^{\iu i} P_i
		= \frac12 D^\m \hat{f}_{\m\n} D^\n 
		+ F_\text{cov}^i K_{i\iu} \bar{F}_\text{cov}^\iu \,,
\end{align*}
which is clearly positive semidefinite and only vanishes
if at least one auxiliary field is non-vanishing.

At a vacuum, the potential must be at a minimum
\begin{align*}%\label{}
%	\frac{\pd V}{\pd \f^j} 
%	&= X_{\m,j}\hat{f}^{\m\n}(\k_\n+X_\n)	
%	+ \frac12(\k_\m+X_\m)\hat{f}_{j}^{\m\n}(\k_\n+X_\n)
%	+ \bar{P}_\iu(K^{\iui}_jP_i+K^\iui P_{ij}) \\
%	X_{\m,j} &= \frac12\big(T_\m{}^i_j K_i + (T_\m\f)^iK_{ij}
%		+(\fb T_\m)^\iu K_{j\iu}\big) 
%	\xlongequal{\d_\m K=0} (\fb T_\m)^\iu K_{j\iu} \\
%		\hat{f}^{\m\n}_j 
%	&= -\hat{f}^{\m\m'}\hat{f}_{\m'\n',j}\hat{f}^{\n'\n} 
%	= -\frac12\hat{f}^{\m\m'} f_{\m'\n',j} \hat{f}^{\n'\n} \\
%	
	\frac{\pd V}{\pd \f^j}  
%	&= -(\fb T_\m)^\iu K_{j\iu}D^\m	- \frac12 D^\m \hat{f}_{\m\n,j}D^\n
%	- F_\text{cov}^i P_{;ij} \\
	&= -\bem P_{;ij} ,& (\fb T_\m)^\iu K_{j\iu} + \frac14 D^\n f_{\n\m,j}\eem
	\cdot \bem F_\text{cov}^i \\ D^\m \eem 
	\xlongequal{\text{VEV}} 0.
\end{align*}
This can be combined with the gauge invariance of the superpotential
\begin{align*}%\label{}
	\d_\m\bar{P} = 0
	\implies (\Fb T_\m)^\iu P_\iu(\F) = 0
	\implies (\fb T_\m)^\iu K_{i\iu}F_\text{cov}^i = 0\,,
\end{align*} 
which we write as
\begin{align*}%\label{}
	\bem(\fb T_\m)^\iu K_{j\iu} + \frac14 D^\r f_{\r\m,j}
	,&  - \frac14 F_\text{cov}^k f_{\m\n,k}\eem
	\cdot \bem F_\text{cov}^j \\ D^\n \eem = 0\,,
\end{align*}
to get the matrix equation
\begin{align}\label{GoldstinoEigenvector-Gauged}
	\bem P_{;ij} & (\fb T_\n)^\iu K_{i\iu} + \frac14 D^\r f_{\r\n,i} \\
		(\fb T_\m)^\iu K_{j\iu} + \frac14 D^\r f_{\r\m,j} 
		& - \frac14 F_\text{cov}^k f_{\m\n,k} \eem
	\bem F_\text{cov}^{j} \\ D^{\n}\eem = 0\ .
\end{align}


This can be compared to the $(\frac12,0)$-fermion mass terms
\begin{align*}%\label{}
	\cL_{m_{1/2}} 
	&= -\frac12(\j^2)^{ij} P_{;ij} 
		+ \frac14\big(-\sqrt2\j^{\a i}f_{\m\n,i}F^\n\l_\a^{\m}
			+ F_\text{cov}^i f_{\m\n,i}(\l^2)^{\m\n}\big)
		- \sqrt2 (\fb\l^\a)^\iu\j_\a^i K_{i\iu} \\
	&= -\frac12 \bem\j^{\a i} ,& \sqrt2 \l^{\a\m}\eem
	\bem P_{;ij} & (\fb T_\n)^\iu K_{i\iu} + \frac14 D^\r f_{\r\n,i} \\
		(\fb T_\m)^\iu K_{j\iu} + \frac14 D^\r f_{\r\m,j} 
		& - \frac14F_\text{cov}^k f_{\m\n,k} \eem
	\bem\j_{\a}^{j} \\ \sqrt2 \l_{\a}^{\n}\eem ,
\end{align*}
So \eqref{GoldstinoEigenvector-Gauged} implies that there exists a massless
fermion that is the Goldstino.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\bibliographystyle{sjtphys} %unsrt
% abbrev = 	Mendeley generated BibTeX with abbreviated journal names.
% others = 	BibTeX file containing references that aren't publications
% 			e.g. code files, Mathematica notebooks, etc...
%\bibliography{abbrev,others} 

\end{document}




